Quantum Satake in type A: part I

We give an interpretation of sl_n webs as morphisms between certain singular Soergel bimodules. We explain how this is a combinatorial, algebraic version of the geometric Satake equivalence (in type A). We then q-deform the construction, giving an equivalence between representations of U_q(sl_n) and certain singular Soergel bimodules for a q-deformed Cartan matrix. In this paper, we discuss the general case but prove only the case n=2,3. In the sequel we will prove the case n >= 4.

==> RepOm.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The fundamental group}
\label{sec-om}
%%%%%%%%%%%%%%%%%%%%%%%%%

%========================
\subsection{Notation, and some equivalent descriptions}
\label{subsec-om-versions}
%========================

\begin{notation} In this paper, $\G$ will always denote a Dynkin diagram, and $\G^\vee$ the Langlands dual Dynkin diagram. These Dynkin diagrams come equipped with their associated root
systems, weight lattices, etcetera. For each $i \in \G$ let $\o_i$ denote the corresponding fundamental weight. Let $G$ (resp. $G^\vee$) denote an algebraic group with Lie algebra $\gg$
(resp. $\gg^\vee$) associated to $\G$ (resp. $\G^\vee$). Write $G_\adj$ or $G_\sc$ for the adjoint or simply-connected algebraic groups for $\G$. Let $\KC = \C((t))$ and $\OC = \C[[t]]$.
\end{notation}

Recall the following standard definition.

\begin{defn} The \emph{fundamental group} $\pi(\G)$ is defined as $\L_{\wt} / \L_{\rt}$, the quotient of the weight lattice by the root lattice. \end{defn}

The fundamental group $\pi(\G)$ is a finite abelian group. Its Pontrjagin dual or character group $\pi(\G)^*$ is also a finite abelian group, non-canonically isomorphic to $\pi(\G)$.

\begin{claim} The following finite abelian groups are all canonically isomorphic, and will be denoted $\Om$.
\begin{itemize}
	\item $\pi(\G^\vee)$.
	\item $\pi(\G)^*$.
	\item $Z(G_{\sc})$, the center of $G_{\sc}$.
	\item $\pi_1(G_{\adj})$.
	\item $\pi_0(G_{\adj}(\KC))$, the component group of $G_{\adj}(\KC)$.
\end{itemize}
\end{claim}

CHECK ME!!!

\begin{proof} This claim is standard. Let us just remark quickly on the isomorphism between $\pi(\G)$ and $Z(G_{\sc})^*$. For each $\l \in \L_{\wt}$ there is a corresponding irreducible
representation $L_\l$, and the action of $G_{\sc}$ on this representation induces a character on $Z(G_{\sc})$. This character is trivial precisely when $\l \in \L_{\rt}$. Because characters
multiply under tensor product, it is easy to see that the map $\L_{\wt} \to Z(G_{\sc})^*$ is a homomorphism. This constructs the isomorphism $\pi(\G) \to \Z(G_{\sc})^*$. \end{proof}

\begin{notation} Let $\tG$ denote the affine Dynkin diagram of $\G$, and let $0$ denote the affine vertex (i.e. choose an embedding $\G \into \tG$). Let $\trmv$ denote the set of vertices
of $\tG$ which can be removed to obtain a diagram isomorphic to $\G$, and let $\rmv = \trmv \cap \G$, so that $\trmv = \rmv \coprod \{0\}$. Note that $\trmv$ is the same as the orbit of $0$
under the automorphism group of $\tG$. \end{notation}

\begin{claim} The set $\trmv$ is in canonical bijection with $\pi(\G)$. That is, it is a $\pi(\G)$-torsor with a distinguished element $0$. There is a map from $\pi(\G)$ to the automorphism
group of $\tG$ which realizes this action of $\pi(\G)$ on $\trmv$. \end{claim}

\begin{proof} For each $i \in \rmv$ one has the corresponding fundamental weight $\o_i \in \L_{\wt}$. To $0 \in \trmv$ we associate the trivial weight $0$. It is known that the fundamental
weights of $\rmv$, together with the zero weight, enumerate a list of coset representatives of $\L_{\wt} / \L_{\rt}$. This was explained to me by Pavel Etingof. \end{proof}

In particular, $\Om$ is in bijection with $\trmv^\vee$, the removable vertices in the dual affine Dynkin diagram.

%========================
\subsection{Monoidal-graded categories}
\label{subsec-om-monoidal}
%========================

\begin{defn} (\cite{ENO}) Let $H$ be a finite abelian group. A monoidal category $\CC$ is $H$-\emph{graded-monoidal} if there are subcategories $\CC_{\xi}$ for $\xi \in H$, for which $\CC =
\oplus_{\xi \in H} \CC_{\xi}$, and for which $\CC_\xi \ot \CC_\nu \subset \CC_{\xi \nu}$. \end{defn}

The category $\Rep = \Rep_{\gg^\vee}$ of finite dimensional $\gg^\vee$ representations is $\Om$-graded-monoidal. For $\xi \in \Om$, let $\Rep_\xi$ denote those representations whose
irreducible constituents all have highest weights in the coset $\xi$, or equivalently, those representations with central character $\xi$ for $Z(G^\vee_{\sc})$. Clearly the tensor product
obeys the group law. From this $\Om$-grading one can reconstruct the category of $G^\vee$ representations for any corresponding algebraic group.

\begin{example} Representations of $\sl_2$ or $SL_2$ can be split into even and odd representations. These can be distinguished by the action of the subgroup $\{ \pm 1 \} \subset SL_2$ on
these representations. The subcategory of even representations is equivalent to the category of $\PM SL_2$-representations. \end{example}

\begin{remark} The adverb $H$-\textbf{graded} modifies the adjective \textbf{monoidal}. One should not confuse this with other uses of the term \textbf{graded}. For instance, a category
is \emph{graded} or \emph{$\Z$-graded} if (by conflating maps of all ``degrees") its Hom spaces can be enriched in graded vector spaces. Therefore, every (homogeneous) \textbf{morphism} has
an associated degree in $\Z$. On the other hand, every (indecomposable) \textbf{object} in an $H$-graded-monoidal category has an associated character in $H$. Eventually, we will be
interested in an $\Om$-graded-monoidal $\Z$-graded category. \end{remark}

\begin{constr} It is a trivial operation to take an $H$-graded-monoidal category and replace it with a $2$-category $\CG$ which encodes (almost) the same data. Let $S$ be a right
$H$-torsor. The objects of $\CG$ will be identified with $s \in S$, and for $\xi \in H$ the morphism category from $s$ to $s \xi$ is $\CC_{\xi}$. A $2$-category where the objects form
an $H$-torsor, equipped with a corresponding $H$ action which identifies $\Hom(s,t) = \Hom(s \xi,t \xi)$, we will call an \emph{$H$-$2$-category}, for lack of better terminology.
\end{constr}

\begin{remark} The data of an $H$-$2$-category $\CG$ together with a choice of $s \in S$ (corresponding to $1 \in H$) and the data of an $H$-graded-monoidal category $\CC$ are equivalent.
Philosophically speaking, the difference between them is analogous to the difference between an algebra and its regular representation. Because $\CC$ is monoidal, it acts on itself by
tensor product. Under the splitting $\CC = \oplus_{\xi \in H} \CC_{\xi}$, the action of $M \ot (\cdot)$ for any object $M$ can be expressed as an $H \times H$ matrix. Each entry of this
matrix is a corresponding 1-morphism in $\CG$. \end{remark}

Thus from $\Rep_{\gg^\vee}$ we can construct an $\Om$-$2$-category which we denote $\RepOm$. One can also construct an $\Om$-$2$-category associated to the
representations of the quantum group $U_q(\gg^\vee)$, which we denote $\RepOmq$.

Why switch from monoidal categories to $2$-categories? Below we shall compare $\RepOm$ to other $2$-categories which do not obviously arise from an $\Om$-graded monoidal category.

\begin{remark} The monoidal category $\Rep_{\gg^\vee}$ has a symmetric structure. There is no notion of a symmetric structure on a $2$-category, but the corresponding structure on an
$\Om$-$2$-category is not hard to formulate. \end{remark}

